Modeling Asymptotic Complexity Using ACL2

The theory of asymptotic complexity provides an approach to characterizing the behavior of programs in terms of bounds on the number of computational steps executed or use of computational resources. We describe work using ACL2 to prove complexity properties of programs implemented in a simple imperative programming language embedding via an operational semantics in ACL2. We simultaneously prove functional properties of a program and its complexity. We illustrate our approach by describing proofs about a binary search algorithm, proving both that it implements binary search on a sorted list and that it is O(log(n)), where n is the length of the list.

==> eptcsdata.tex <==
\providecommand{\firstpage}{83}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.9}{10.4204/EPTCS.359.9}}
\pdfoutput=1

